Bayesian Filtering in Physical Systems via Test-time Trained Flow Matching

Bayesian filtering provides a principled framework for online state estimation under uncertainty, yet its application to systems with high-dimensional states and complicated posterior distributions remains challenging. Recent generative models, such as flow matching, have shown potential in Bayesian filtering. However, they still rely on particle-based representations of the posterior, which lose the rich information of the full distribution, or tackle a trajectory-level inverse problem that conflicts with the recursive structure of Bayesian filtering. To address this, we propose a new perspective of directly encoding the evolving distribution into flow matching model weights, namely, the Belief Flow Filter (BFF). It is a generative filtering framework that updates model weights via gradient descent at test time to track the posterior evolution. Thereby, BFF bypasses the scalability issue of particle representations or the flexibility limitation of Gaussian assumptions in conventional filters. We theoretically justify that the BFF design is structurally aligned with Bayesian filtering, and its training objective targets the recursive filtering operator. BFF is empirically verified across 5 different physical systems, including ones with chaotic dynamics and highly sparse, non-linear observations. The results show that BFF attains the best score in 8 of 9 metric-benchmark cells across the three standard 1D and 2D PDE benchmarks, and similarly leads on the extreme single-moving-sensor setting and on a real-world-grounded tokamak plasma estimation task, demonstrating its potential to accurately approximate the Bayesian filtering operator in high-dimensional probability space.

==> tables/single_sensor.tex <==
\begin{table}[t]
\centering
\small
\caption{\textbf{2D Navier-Stokes with a single moving sensor.} A single sensor traverses the flow field along a pre-defined scan trajectory, compressing each $128\!\times\!128$ velocity snapshot into one scalar measurement ($16384\!:\!1$ compression ratio). This setup breaks the fixed uniform-grid assumption commonly adopted in neural data-assimilation work. \textbf{Bold} denotes the best and \underline{underline} denotes the second best.}
\label{tab:single_sensor}
\setlength{\tabcolsep}{18pt}
\begin{tabular}{@{}lcc@{}}
\toprule
\textbf{Method} & $\mathcal{E}_{L_2}\!\downarrow$ & $\mathcal{E}_{\mathrm{spec}}\!\downarrow$ \\
\midrule
POD-LKF~\citep{willcox2006unsteady}     & \underline{$0.5910$} & $0.5845$ \\
FNO-EnKF~\citep{li_fourier_2021,evensen2009sequential} & $0.7859$ & \underline{$0.0642$} \\
Transformer~\citep{vaswani_attention_2017} & $0.7516$ & $0.2767$ \\
\ourmethod (ours)                       & $\mathbf{0.3771}$ & $\mathbf{0.0286}$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/tkmk1.tex <==
\begin{table}[tb]
\centering
\small
\caption{\textbf{Comprehensive quantitative results for tokamak plasma profile estimation.} We report the relative $L_2$ error ($\mathcal{E}_{L_2}$), gradient relative $L_2$ error ($\mathcal{E}_{\mathrm{grad}}$), and spectrum deviation ($\mathcal{E}_{\mathrm{spec}}$) across three key physical variables: $T_e$, $\psi_{axis}$, and $n_e$. \textbf{Bold} denotes the best and \underline{underline} denotes the second best.}
\label{table:tkmk1} % 已将 label 移至 caption 之下以防引用报错
% 自动缩放以适应页面单栏宽度
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{$T_e$}} & \multicolumn{3}{c}{\textbf{$\psi_{axis}$}} & \multicolumn{3}{c}{\textbf{$n_e$}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
 & $\mathcal{E}_{L_2}\!\!\downarrow$ & $\mathcal{E}_{\mathrm{grad}}\!\!\downarrow$ & $\mathcal{E}_{\mathrm{spec}}\!\!\downarrow$ & $\mathcal{E}_{L_2}\!\!\downarrow$ & $\mathcal{E}_{\mathrm{grad}}\!\!\downarrow$ & $\mathcal{E}_{\mathrm{spec}}\!\!\downarrow$ & $\mathcal{E}_{L_2}\!\!\downarrow$ & $\mathcal{E}_{\mathrm{grad}}\!\!\downarrow$ & $\mathcal{E}_{\mathrm{spec}}\!\!\downarrow$ \\
\midrule
EKF & 0.0719 & 0.1166 & 0.0669 & 0.0584 & 0.0542 & 0.0922 & 0.1745 & 0.3263 & 0.4658 \\
EnKF & 0.0666 & 0.0846 & \textbf{0.0035} & 0.0330 & 0.0315 & 0.0559 & 0.1615 & 0.2460 & 0.4666 \\
FNO-EnKF & 0.1303 & 3.6560 & 0.1250 & 0.1280 & 2.3260 & 0.1696 & 0.1724 & 0.3279 & 0.4067 \\
POD-LKF & 0.0675 & 0.0906 & 0.0153 & 0.0352 & 0.0336 & 0.0596 & 0.1426 & 0.2539 & 0.3966 \\
\midrule
FNO & 0.0145 & \underline{0.0802} & 0.0049 & 0.0080 & 0.0394 & \underline{0.0025} & 0.0297 & 0.1141 & 0.0301 \\
CNN & \underline{0.0144} & 0.1361 & 0.0061 & \underline{0.0078} & 0.0566 & 0.0045 & \underline{0.0288} & 0.1493 & 0.0364 \\
\midrule
SDA & 0.3984 & 1.2630 & 1.0570 & 0.1911 & 0.5181 & 0.2248 & 0.2926 & 1.0640 & 0.0377 \\
FlowDAS & 0.0618 & 0.1258 & 0.0167 & 0.0255 & \underline{0.0272} & 0.0026 & \textbf{0.0026} & \textbf{0.0213} & \textbf{0.0031} \\
\midrule
\ourmethod (ours) & \textbf{0.0124} & \textbf{0.0409} & \underline{0.0045} & \textbf{0.0065} & \textbf{0.0071} & \textbf{0.0004} & 0.0338 & \underline{0.0828} & \underline{0.0114} \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex/results/2_uq.tex <==
\label{sec:uq}

\ourmethod captures multi-modal posteriors. In the 4-sensor Burgers' setting, the lack of spatial observation near the shock front leads to high uncertainty regarding the exact shock location. Because of the abrupt state transition across the wavefront, the marginal posterior at the shock interface naturally exhibits a bimodal distribution, representing a probabilistic mixture of pre-shock and post-shock states. As shown in Figure~\ref{fig:bimodal_visualizations}(a), our method accurately recovers this complex statistical feature.
We assess the full posterior at the distribution level: a distributionally accurate Bayesian filter must minimize tracking error \emph{and} provide calibrated uncertainty. Using the miscalibration measure of~\citet{chung_uncertainty_2021},
\begin{equation}
\mathbb{E}_{s_t,h_t\sim P_{\text{data}}}\big[|p(s_t \in Q \mid h_t) - q|\big],
\end{equation}
where $Q$ is the model confidence interval at promised coverage $q$, we compute the Miscalibration Area (MA) by averaging over $q$, with $Q$ endpoints from the $\frac{1\mp q}{2}$ sample quantiles of an ensemble of $16$ samples. As shown in Figure~\ref{fig:diagnostic_metrics}(b), \ourmethod attains consistently low MA, while other baselines exhibit significant over- or under-confidenceconfirming that our framework approximates the high-dimensional posterior $b_t$.




==> tex/results/4_generalize.tex <==
% \label{sec:generalization}

% To test whether \ourmethod has learned the underlying filtering operator rather than memorizing a fixed horizon,

==> tex/results/5_nonlinear_obs.tex <==
% Deprecated: content moved to Appendix~\ref{app:tokamak} (Tokamak setup, table, figure)
% and Appendix~\ref{app:dataset} (single-moving-sensor scan setup).
% This file is no longer included from main.tex and is kept only as a placeholder.

